Approximately Stable, School Optimal, and Student-Truthful Many-to-One Matchings (via Differential Privacy)

We present a mechanism for computing asymptotically stable school optimal matchings, while guaranteeing that it is an asymptotic dominant strategy for every student to report their true preferences to the mechanism. Our main tool in this endeavor is differential privacy: we give an algorithm that coordinates a stable matching using differentially private signals, which lead to our truthfulness guarantee. This is the first setting in which it is known how to achieve nontrivial truthfulness guarantees for students when computing school optimal matchings, assuming worst- case preferences (for schools and students) in large markets.

==> lowerbdd.tex <==
\section{Lower Bounds}
We show that it is impossible for private mechanisms to have the
matchings as the output (i.e., $\cR = U^n$). In other words, in order
to preserve privacy, the algorithm cannot publish the final
matching. Intuitively, publishing a stable matching reveals quite a
lot about each student's private preferences, if a student has a
reasonable chance of being assigned to her more-preferred school
subject to available space. A full proof of the following theorem can
be found in Appendix~\ref{lowerbdd}.

\begin{restatable}{theorem}{dplower}
  \label{thm:dplower}
  Suppose $\cM \colon (\cP\times \cV)^n \rightarrow U^n$ satisfies
  $\eps$-differential privacy. Then on a class of $n$ student
  profiles, $\cM$ would produce $\Omega(n/\eps)$ blocking empty seats
  with probability at least $\displaystyle 1/\left({1 +
      \exp(2\eps)}\right)$.
\end{restatable}
\jmcomment{Make sure this number is right}

